An Integral Field Spectroscopy Study Of Thin And Thick Discs In IC 2531

Thin and thick discs are prominent components in the Milky Way and other spiral galaxies, but their formation histories are not yet understood, which is particularly true for thick discs. This is partially due to the fact that we lack sufficient understanding of thin and thick discs in other galaxies to determine how common features of the Milky Way's discs are. Here, we conduct an integral field spectroscopy study of the thin and thick discs in the edge-on Milky Way analogue IC 2531, using observational data from the WiFeS IFU spectrograph on the ANU 2.3m telescope. We provide spectral analysis of IC 2531's kinematics and stellar populations in the thin and thick disc regions by conducting pPXF fitting with Vazdekis models. We found that IC 2531's disc above the dust plane generally has chemical properties between the Milky Way's chemical thin and thick disc. IC 2531's thick disc is somewhat similar to the Milky Way's in terms of stellar populations: on average, it is older, more metal-poor than its corresponding thin disc, but similarly alpha-enhanced in general. But we do find a clearly alpha-rich thick disc bin though one of our "thick disc" bins may be dominated by a warped thin disc. These results may help to constrain formation theories of thick discs.

==> references.tex <==


\bibitem[\protect\citeauthoryear{van de Sande et al.}{2024}]{2024IAUS..377...27V} van de Sande J., Fraser-McKelvie A., Fisher D.~B., Martig M., Hayden M.~R., Geckos Survey Collaboration, 2024, IAUS, 377, 27. doi:10.1017/S1743921323001138

